An Assessment of Solvers for Algebraically Stabilized Discretizations of Convection-Diffusion-Reaction Equations

We consider flux-corrected finite element discretizations of 3D convection-dominated transport problems and assess the computational efficiency of algorithms based on such approximations. The methods under investigation include flux-corrected transport schemes and monolithic limiters. We discretize in space using a continuous Galerkin method and $\mathbb{P}_1$ or $\mathbb{Q}_1$ finite elements. Time integration is performed using the Crank-Nicolson method or an explicit strong stability preserving Runge-Kutta method. Nonlinear systems are solved using a fixed-point iteration method, which requires solution of large linear systems at each iteration or time step. The great variety of options in the choice of discretization methods and solver components calls for a dedicated comparative study of existing approaches. To perform such a study, we define new 3D test problems for time-dependent and stationary convection-diffusion-reaction equations. The results of our numerical experiments illustrate how the limiting technique, time discretization and solver impact on the overall performance.

==> graphs/rotating_shapes/rotating_shapes.tex <==
This example of a time-dependent problem compares the precision of the monolithic limiter with that of Zalesak's limiter. It is meant as an analogy to the famous 2D example with rotating shapes in \cite{Le96}. To the best of our knowledge, a similar comparison in 3D has not been reported before.

We consider the problem \eqref{eq:tcdr} with $\Omega = (0,1)^3$, $\varepsilon = 10^{-20}$, $\bfb = (0.5 - y, x-0.5, 0)^\text{T}$, $\sigma = 0$, $f = 0$, $T=2\pi$ and homogeneous Dirichlet boundary conditions on the whole of $\Omega$. The initial condition $u_0$ is depicted in Figure \ref{fig:ini_rotating_shapes}, i.e., $u_0$ takes the value 1 in the volumes enclosed by the red surfaces and zero everywhere else. These volumes have the following properties:
\begin{itemize}
    \item cube: faces parallel to the coordinate axes, center at $(0.5, 0.25, 0.5)^\text{T}$ and edges of the length 0.25;
    \item cone: bottom face with the radius 0.125 and center at $(0.75, 0.5,0.25)^\text{T}$ parallel to the coordinate axes and height 0.5;
    \item hollow cylinder: upper and bottom faces parallel to the coordinate axes, inner radium 0.0625, outer radius 0.125, height 0.5, bottom face having its center at $(0.5, 0.75, 0.25)^\text{T}$.
\end{itemize}
The above flow field $\bfb$ makes the spatial shapes rotate about the axis given by $x=y=0.5$, where the time needed for one full turn is $T=2\pi$. Thus, the true solution satisfies $u(T, \bfx) = u_0(\bfx)$ $\forall \bfx \in \Omega$.

Our simulations were carried out using the uniform mesh of cubes with the edge of the length $2^{-8}$ and the time step $10^{-3}$. The systems of linear algebraic equations arising in the schemes using Zalesak's limiter were solved via the solver LGMRES with the Jacobi preconditioner and the default setup.

Figures \ref{fig:ini_rotating_shapes_slice}--\ref{fig:monolithic_rotating_shapes_slice} show the resulting $u(T, \bfx)$ and $u_0(\bfx)$ for $\bfx$ in a plane given by $z=0.5$. We can see that the results of the monolithic limiter are better than those of the schemes based on Zalesak's limiter, although they are also smeared. Note that contrary to Zalesak's limiter, the smearing performed by the monolithic limiter is somewhat uniform. The superiority of the monolithic limiter in this test can be also illustrated by Figure \ref{fig:rotating_shapes_point} that depicts the time evolution of the solution at the point $0.5, 0.25, 0.5$ (i.e., initial center of the cube).

We want to point out that none of the schemes produced values of $u$ larger than 1 or lower than 0, as expected.

\begin{figure}
\centering
\includegraphics[width=\textwidth, trim = 3cm 4cm 10cm 7cm, clip = true]
{./graphs/rotating_shapes/initial_condition.png}
\caption{Initial condition}
\label{fig:ini_rotating_shapes}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.49\textwidth, trim = 2.5cm 6cm 4cm 2cm, clip = true]
{./graphs/rotating_shapes/initial_condition_slice2.png}\
\includegraphics[width=0.49\textwidth, trim = 2.5cm 6cm 4cm 2cm, clip = true]
{./graphs/rotating_shapes/linear_end_slice2.png}
\includegraphics[width=0.49\textwidth, trim = 2.5cm 6cm 4cm 2cm, clip = true]
{./graphs/rotating_shapes/nonlinear_c_end_slice2.png}\
\includegraphics[width=0.49\textwidth, trim = 2.5cm 6cm 4cm 2cm, clip = true]
{./graphs/rotating_shapes/monolithic_end_slice2.png}
\caption{Initial condition $u_0(\bfx)$ for $\bfx$ in plane $z=0.5$.}
\label{fig:ini_rotating_shapes_slice}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\textwidth, trim = 3cm 7cm 4cm 2cm, clip = true]
{./graphs/rotating_shapes/linear_end_slice.png}
\caption{Solution $u(T, \bfx)$ for $\bfx$ in plane $z=0.5$ calculated by using the linearized version of Zalesak's limiter.}
\label{fig:linear_rotating_shapes_slice}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\textwidth, trim = 3cm 7cm 4cm 2cm, clip = true]
{./graphs/rotating_shapes/nonlinear_c_end_slice.png}
\caption{Solution $u(T, \bfx)$ for $\bfx$ in plane $z=0.5$ calculated by using the nonlinear version of Zalesak's limiter with the stopping tolerance $4 \cdot 10^{-12}$ for the residual in the nonlinear loop.}
\label{fig:nonlinear_rotating_shapes_slice}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\textwidth, trim = 3cm 7cm 4cm 2cm, clip = true]
{./graphs/rotating_shapes/monolithic_end_slice.png}
\caption{Solution $u(T, \bfx)$ for $\bfx$ in plane $z=0.5$ calculated by using the monolithic limiter.}
\label{fig:monolithic_rotating_shapes_slice}
\end{figure}

\begin{figure}
\centerline{\input{./graphs/rotating_shapes/rotating_shapes_point.tex}}
\caption{Time evolution of the numerical solution and true solution at point $(0.5, 0.25, 0.5)$ (i.e., initial center of the cube). We can also see that the stopping tolerance for the residual in the nonlinear loop of the scheme with the nonlinear Zalesak's limiter should be chosen very carefully.}
\label{fig:rotating_shapes_point}
\end{figure}


==> tables/bjkr18_BJK17_seqParTable.tex <==
\begin{table}[!ht]
\centering
\caption{Example~\ref{ex:non_constant_convection2}: Computing times in seconds of the solver with the LP limiter for refinement level 3.}
\begin{tabular}{c c c c c c c c }
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{time (sec)}}&\multicolumn{2}{c}{} &\multicolumn{2}{c}{\textbf{time (sec)}}\\ 
\textbf{Solver} & \textbf{PC} & NP = 1 & NP=4 & \textbf{Solver} & \textbf{PC} & NP = 1 & NP = 4\\ \midrule
\multirow{4}{*}{LGMRES} & BJac & 56.7 & 19.0 & \multirow{3}{*}{BCGS} & BJac   & 55.3 & 18.4 \\ \cline{2-4} \cline{6-8}
 & SOR  & 60.1 & ---  & & SOR    & 58.2 & --- \\ \cline{2-4} \cline{6-8}
 & ASM  & 59.2 & 18.1 & & ASM    & 57.8 & 19.4 \\ \cline{2-4} \cline{5-8}
 & Jac  & 81.1 & 24.5 & &     &     &     \\ \midrule
\multirow{4}{*}{FGMRES} & BJac & 42.1 & 14.3 & & & & \\ \cline{2-4} \cline{5-8}
 & SOR  & 44.0 & 15.3 & & & &\\ \cline{2-4} \cline{5-8}
 & ASM  & 43.8 & 15.1 & & & &\\ \cline{2-4} \cline{5-8}
 & Jac  & 59.8 & 18.7 & & & &\\ 
\end{tabular}
\label{tab:bjkr18_BJK17}
\end{table}


==> tables/bjkr18_kuzmin_seqParTable.tex <==
\begin{table}[!ht]
\centering
\caption{Example~\ref{ex:non_constant_convection2}: Computing times in seconds of the solver with the MU limiter for refinement level 3.}
\begin{tabular}{c c c c c c c c}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{time (sec)}}&\multicolumn{2}{c}{} &\multicolumn{2}{c}{\textbf{time (sec)}}\\
\textbf{Solver} & \textbf{PC} & NP = 1 & NP=4 & \textbf{Solver} & \textbf{PC} & NP = 1 & NP = 4\\ \midrule
\multirow{4}{*}{LGMRES} & BJac & 7.5 & 2.5 & \multirow{3}{*}{BCGS} & BJac & 7.8 & 2.7 \\ \cline{2-4} \cline{6-8}
 & SOR    & 7.7 & --- & & SOR & 7.7 & --- \\ \cline{2-4} \cline{6-8}
 & ASM    & 7.7 & 2.7 & & ASM & 7.8 & 2.8 \\ \cline{2-4} \cline{5-8}
 & Jac    & 9.2 & 3.0 & &     &     &     \\ \midrule
\multirow{4}{*}{FGMRES} & BJac & 6.7 & 2.3 & & & & \\ \cline{2-4} \cline{5-8}
 & SOR    & 6.8 & 2.4 & & & &\\ \cline{2-4} \cline{5-8}
 & ASM    & 6.9 & 2.5 & & & &\\ \cline{2-4} \cline{5-8}
 & Jac    & 7.9 & 2.6 & & & &\\ 
\end{tabular}
\label{tab:bjkr18_kuzmin}
\end{table}


==> tables/bjkr18_monolithic_seqParTable.tex <==
\begin{table}[!ht]
\centering
\caption{Example~\ref{ex:non_constant_convection2}: Computing times in seconds of the solver with the MC limiter for refinement level 3.}
\begin{tabular}{c c c c c c c c }
\multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{time (sec)}}&\multicolumn{2}{c}{} &\multicolumn{2}{c}{\textbf{time (sec)}}\\
\textbf{Solver} & \textbf{PC} & NP = 1 & NP=4 & \textbf{Solver} & \textbf{PC} & NP = 1 & NP = 4\\ \midrule
\multirow{4}{*}{LGMRES} & BJac & 5.3 & 2.1 & \multirow{3}{*}{BCGS} & BJac   & 5.3 & 2.1 \\ \cline{2-4} \cline{6-8}
 & SOR  & 5.4 & --- & & SOR    & 5.3 & --- \\ \cline{2-4} \cline{6-8}
 & ASM  & 5.5 & 2.1 & & ASM    & 5.4 & 2.3 \\ \cline{2-4} \cline{5-8}
 & Jac  & 6.5 & 2.4 & &     &     &     \\ \midrule
\multirow{4}{*}{FGMRES} & BJac & 4.7 & 1.9 & & & & \\ \cline{2-4} \cline{5-8} 
 & SOR  & 4.6 & 1.9 & & & &\\ \cline{2-4} \cline{5-8}
 & ASM  & 4.7 & 1.9 & & & &\\ \cline{2-4} \cline{5-8}
 & Jac  & 5.4 & 2.1 & & & &\\
\end{tabular}
\label{tab:bjkr18_monolithic}
\end{table}


==> tables/linear_sequential.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c c|c|c|c c|}
\hline
\multicolumn{2}{|c}{} & \multicolumn{2}{c}{\textbf{time (sec)}}&\multicolumn{2}{c}{} &\multicolumn{2}{c|}{\textbf{time (sec)}}\\ \hline
\textbf{Solver} & \textbf{PC} & NP = 1 & NP=4 & \textbf{Solver} & \textbf{PC} & NP = 1 & NP = 4\\ \hline \hline
\multirow{5}{*}{BCGS} & BJac & 1,232  & 421  & \multirow{5}{*}{FGMRES} & BJac  & 1,221  & 418 \\ \cline{2-4} \cline{6-8}
 & SOR & 1,243  & 417  &  & SOR   & 1,228  & 414 \\ \cline{2-4} \cline{6-8}
 & ASM & 1,264  & 436  &  & ASM   & 1,264  & 431 \\ \cline{2-4} \cline{6-8}
 & Jac & 1,237  & ---  &  & Jac   & 1,210  & 408 \\ \cline{2-4} \cline{6-8}
 & MG   & 1,270 & 434  &  & MG    & 1,251  & 422 \\ \hline
\multirow{5}{*}{LGMRES} & BJac  & 1,244  & 421  & LU &  & 4,934  & 2,540   \\ \cline{2-4} \cline{5-8}
 & SOR   & 1,228  & 423  & UMFPACK & & 1,221  & 2,562   \\ \cline{2-4} \cline{5-8}
 & ASM   & 1,257  & 441 & & & &\\ \cline{2-4} \cline{5-8}
 & Jac   & 1,220  & 409 & & & &\\ \cline{2-4} \cline{5-8}
 & MG    & 1,263  & 438 & & & &\\ \hline
\end{tabular}
\caption{Example~\ref{ex:concentration_species2}: Linear Zal+CN: Computing time in seconds for $\text{NP} = 1, 4$ and refinement level 5.}
\label{tab;linear_sequential}
\end{table}


==> tables/monolithic.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
 & \multicolumn{3}{|c|}{time (s)}\\ \hline
 & \multicolumn{3}{|c|}{refinement level}\\ \hline
np & 5 & 6 & 7         \\ \hline \hline
1 & 3,450  & --- & ---              \\ \hline
4 & 1,083 &  7,950 & 62,611               \\ \hline
8 & 591   &  4,215 & 32,496               \\ \hline
16 & 392  & 2,394 & 17,227                \\ \hline
32 & 248 &  1,399 & 9,468                 \\ \hline
\end{tabular}
\caption{Monolithic sequential and MPI.}
\label{tab;monolithic}
\end{table}


==> tables/nonlinear_sequential.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c| c c|c|c|c c|}
\hline
\multicolumn{2}{|c}{} & \multicolumn{2}{c}{\textbf{time (sec)}}&\multicolumn{2}{c}{} &\multicolumn{2}{c|}{\textbf{time (sec)}}\\ \hline
\textbf{Solver} & \textbf{PC} & NP = 1 & NP=4 & \textbf{Solver} & \textbf{PC} & NP = 1 & NP = 4\\ \hline \hline
\multirow{5}{*}{BCGS} & BJac & 2,023 & 727 & \multirow{5}{*}{FGMRES} & BJac & 1,988 & 708 \\ \cline{2-4} \cline{6-8}
 & SOR & 1,961        & 712 &  & SOR & 1,921 & 694 \\ \cline{2-4} \cline{6-8}
 & ASM & 2,093        & 789 &  & ASM & 2,095 & 781 \\ \cline{2-4} \cline{6-8}
 & Jac & 1,947        & --- &  & Jac & 1,913 & 685 \\ \cline{2-4} \cline{6-8}
 & MG &  2,112        & 776 &  & MG &  2,036 & 735 \\ \hline
\multirow{5}{*}{LGMRES} & BJac & 2,015 & 725 & LU & & 16,905 & 9,152 \\ \cline{2-4} \cline{5-8}
 & SOR & 1,962      & 708 & UMFPACK & & 1,968 & 9,248 \\ \cline{2-4} \cline{5-8}
 & ASM & 2,131      & 780 & & & & \\ \cline{2-4} \cline{5-8}
 & Jac & 1,949      & 701 & & & & \\ \cline{2-4} \cline{5-8}
 & MG &  2,102      & 767 & & & & \\ \hline
\end{tabular}
\caption{Example~\ref{ex:concentration_species2}: Nonlinear Zal+CN: Computing time in seconds for $\text{NP} = 1, 4$ and refinement level 5.}
\label{tab;nonlinear_sequential}
\end{table}


==> tables/smooth_solution_3d_H1_precTable.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
level & monolithic & BJK17 & kuzmin & plain FEM \\ \hline
5 & 1.07e-02 & 2.80e-03 & 3.74e-03 & 3.37e-02 \\ \hline
6 & 6.10e-03 & 1.35e-03 & 2.16e-03 & 3.36e-02 \\ \hline
7 & 3.24e-03 & 6.72e-04 & 1.35e-03 & 6.72e-04 \\ \hline
\end{tabular}
\caption{Error measured in $\left\arrowvert \cdot \right\arrowvert_1$.}
\label{tab:smooth_solution_3d_H1}
\end{table}


==> tables/smooth_solution_3d_L2_precTable.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
level & monolithic & BJK17 & kuzmin & plain FEM \\ \hline
5 & 4.29e-04 & 1.74e-05 & 6.54e-05 & 6.09e-03 \\ \hline
6 & 1.99e-04 & 4.14e-06 & 2.14e-05 & 6.09e-03 \\ \hline
7 & 8.80e-05 & 1.02e-06 & 7.86e-06 & 9.76e-07 \\ \hline
\end{tabular}
\caption{Error measured in $\left\Arrowvert \cdot \right\Arrowvert$.}
\label{tab:smooth_solution_3d_L2}
\end{table}


==> tables/smooth_solution_3d_Linf_L2_H1_precTable.tex <==
\begin{table}
\begin{subtable}{\textwidth}
\centering
\begin{tabular}{|c c c c c|}
\hline
\textbf{Level} & \textbf{MC} & \textbf{LP} & \textbf{MU} & \textbf{Plain FEM} \\ \hline\hline
5 & 1.07e-02 & 2.80e-03 & 3.74e-03 & 3.37e-02 \\ \hline
6 & 6.10e-03 & 1.35e-03 & 2.16e-03 & 3.36e-02 \\ \hline
7 & 3.24e-03 & 6.72e-04 & 1.35e-03 & 6.72e-04 \\ \hline
\end{tabular}
\caption{Error measured in $\left\arrowvert \cdot \right\arrowvert_1$.}
\label{tab:smooth_solution_3d_H1}
\end{subtable}
\par\bigskip
\begin{subtable}{\textwidth}
\centering
\begin{tabular}{|c c c c c|}
\hline
\textbf{Level} & \textbf{MC} & \textbf{LP} & \textbf{MU} & \textbf{Plain FEM} \\ \hline\hline
5 & 4.29e-04 & 1.74e-05 & 6.54e-05 & 6.09e-03 \\ \hline
6 & 1.99e-04 & 4.14e-06 & 2.14e-05 & 6.09e-03 \\ \hline
7 & 8.80e-05 & 1.02e-06 & 7.86e-06 & 9.76e-07 \\ \hline
\end{tabular}
\caption{Error measured in $\left\Arrowvert \cdot \right\Arrowvert$.}
\label{tab:smooth_solution_3d_L2}
\end{subtable}
\par\bigskip
\begin{subtable}{\textwidth}
\centering
\begin{tabular}{|c c c c c|}
\hline
\textbf{Level} & \textbf{MC} & \textbf{LP} & \textbf{MU} & \textbf{Plain FEM} \\ \hline\hline
5 & 1.05e-03 & 1.74e-04 & 3.77e-04 & 1.56e-02 \\ \hline
6 & 4.62e-04 & 3.49e-05 & 1.82e-04 & 1.56e-02 \\ \hline
7 & 1.93e-04 & 5.95e-06 & 8.72e-05 & 5.95e-06 \\ \hline
\end{tabular}
\caption{Error measured in $\left\Arrowvert \cdot \right\Arrowvert_\infty$.}
\label{tab:smooth_solution_3d_Linf}
\end{subtable}
\caption{Example~\ref{ex:smooth_solution}: Errors in different norms.}
\label{tab:smooth_solution_3d_errors}
\end{table}


==> tables/smooth_solution_3d_Linf_precTable.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
level & monolithic & BJK17 & kuzmin & plain FEM \\ \hline
5 & 1.05e-03 & 1.74e-04 & 3.77e-04 & 1.56e-02 \\ \hline
6 & 4.62e-04 & 3.49e-05 & 1.82e-04 & 1.56e-02 \\ \hline
7 & 1.93e-04 & 5.95e-06 & 8.72e-05 & 5.95e-06 \\ \hline
\end{tabular}
\caption{Error measured in $\left\Arrowvert \cdot \right\Arrowvert_\infty$.}
\label{tab:smooth_solution_3d_Linf}
\end{table}

